Revival of the Reactor Antineutrino Anomaly

The Reactor Antineutrino Anomaly (RAA) refers to the deficit observed between the average event rate measured in reactor antineutrino experiments with respect to the theoretical prediction. This anomaly was first identified in 2011 ($2.5\,\sigma$) as a consequence of the Huber-Muller reactor antineutrino flux calculation. It was thought to be resolved in 2021 as a result of previous reactor antineutrino flux calculations, with a reduction to about $1\,\sigma$. In this work, we present the RAA obtained with the latest reactor antineutrino flux calculation published in 2023 by a French research group, which was never used before for the calculation of the RAA. It is the first summation flux model which includes a comprehensive uncertainty budget. The result indicates a revival of the RAA at the level of $2.2\,\sigma$. We also consider the usual simplest explanation of the RAA by active-sterile neutrino oscillations. We present the constraints on the oscillation parameters and we derive a tension of $3.8\,\sigma$ with the results of gallium source experiments (Gallium Anomaly) taking into account also the solar neutrino and KATRIN bounds, that of the combined short-baseline reactor spectral ratio measurements, and that of the Daya Bay search for a sub-eV sterile neutrino. Since the tension may be due to underestimated systematic uncertainties and the main tension is between the gallium data and the other data, we finally present the results of a global analysis with enlarged gallium uncertainties, which reduce the global tension to $1.3\,\sigma$.

==> tables/tab-dev.tex <==
\begin{tabular}{l|c|c|c|c|c|c|c}
\bf Model (M)
&
$\bm{r_{235}-1}$
&
$\bm{r_{238}-1}$
&
$\bm{r_{239}-1}$
&
$\bm{r_{241}-1}$
&
$\bm{\chi^2_{\text{the}}}$
&
$\bm{\chi^2_{\text{exp}}}$
&
$\bm{\Delta\chi^2}$
\\
\hline
\bf HM
&
$-0.0580$
&
$-0.0976$
&
$-0.0664$
&
$-0.0590$
&
$6.78$
&
$16.49$
&
$6.79$
\\
\bf EF
&
$-0.0005$
&
$-0.1260$
&
$-0.0491$
&
$-0.0116$
&
$2.61$
&
$18.95$
&
$1.42$
\\
\bf KI
&
$-0.0213$
&
$-0.0511$
&
$-0.0306$
&
$-0.0255$
&
$2.10$
&
$21.09$
&
$1.40$
\\
\bf CEA
&
$-0.0097$
&
$-0.0332$
&
$-0.0606$
&
$-0.0148$
&
$4.74$
&
$23.58$
&
$5.02$
\end{tabular}


==> tables/tab-rex-norefs.tex <==
\begin{tabular}{clcccccccc}
$a$
&
Experiment
&
$f^{a}_{235}$
&
$f^{a}_{238}$
&
$f^{a}_{239}$
&
$f^{a}_{241}$
&
$\sigma_{f,a}^{\text{exp}}$
&
$\delta_{a}^{\text{exp}}$ [\%]
&
$\delta_{a}^{\text{cor}}$ [\%]
&
$L_{a}$ [m]
\\
\toprule
$1$	&Bugey-4	&$0.538$	&$0.078$	&$0.328$	&$0.056$	&$5.750\pm0.084$	&$1.4$	&\rdelim\}{2}{20pt}[1.4]	&$15$\\
$2$	&Rovno91	&$0.614$	&$0.074$	&$0.274$	&$0.038$	&$5.850\pm0.170$	&$2.8$	&                       	&$18$\\
\midrule
$3$	&Rovno88-1I	&$0.607$	&$0.074$	&$0.277$	&$0.042$	&$5.700\pm0.387$	&$6.4$	&\rdelim\}{2}{20pt}[3.1] \rdelim\}{5}{20pt}[2.2]	&$18.0$\\
$4$	&Rovno88-2I	&$0.603$	&$0.076$	&$0.276$	&$0.045$	&$5.890\pm0.387$	&$6.4$	&                                               	&$17.96$\\
$5$	&Rovno88-1S	&$0.606$	&$0.074$	&$0.277$	&$0.043$	&$6.040\pm0.444$	&$7.3$	&\rdelim\}{3}{45pt}[3.1]                        	&$18.15$\\
$6$	&Rovno88-2S	&$0.557$	&$0.076$	&$0.313$	&$0.054$	&$5.960\pm0.440$	&$7.3$	&                                               	&$25.17$\\
$7$	&Rovno88-3S	&$0.606$	&$0.074$	&$0.274$	&$0.046$	&$5.830\pm0.410$	&$6.8$	&                                               	&$18.18$\\
\midrule
$8$	&Bugey-3-15	&$0.538$	&$0.078$	&$0.328$	&$0.056$	&$5.772\pm0.251$	&$4.2$	&\rdelim\}{3}{20pt}[4.0]                        	&$15$\\
$9$	&Bugey-3-40	&$0.538$	&$0.078$	&$0.328$	&$0.056$	&$5.809\pm0.257$	&$4.3$	&                                               	&$40$\\
$10$	&Bugey-3-95	&$0.538$	&$0.078$	&$0.328$	&$0.056$	&$5.345\pm0.909$	&$15.2$	&                                               	&$95$\\
\midrule
$11$	&Gosgen-38	&$0.619$	&$0.067$	&$0.272$	&$0.042$	&$5.989\pm0.326$	&$5.4$	&\rdelim\}{3}{20pt}[2.0] \rdelim\}{4}{20pt}[3.8]	&$37.9$\\
$12$	&Gosgen-46	&$0.584$	&$0.068$	&$0.298$	&$0.050$	&$6.090\pm0.324$	&$5.4$	&                                               	&$45.9$\\
$13$	&Gosgen-65	&$0.543$	&$0.070$	&$0.329$	&$0.058$	&$5.615\pm0.399$	&$6.7$	&                                               	&$64.7$\\
$14$	&ILL	&$1.000$	&$0$	&$0$	&$0$	&$5.301\pm0.569$	&$9.1$	&                                               	&$8.76$\\
\midrule
$15$	&Krasnoyarsk87-33	&$1.000$	&$0$	&$0$	&$0$	&$6.200\pm0.323$	&$5.2$	&\rdelim\}{2}{20pt}[4.1]	&$32.8$\\
$16$	&Krasnoyarsk87-92	&$1.000$	&$0$	&$0$	&$0$	&$6.300\pm1.280$	&$20.5$	&                       	&$92.3$\\
$17$	&Krasnoyarsk94-57	&$1.000$	&$0$	&$0$	&$0$	&$6.260\pm0.260$	&$4.2$	&0                      	&$57.3$\\
$18$	&Krasnoyarsk99-34	&$1.000$	&$0$	&$0$	&$0$	&$6.390\pm0.186$	&$3.0$	&0                      	&$34.0$\\
\midrule
$19$	&SRP-18	&$1.000$	&$0$	&$0$	&$0$	&$6.293\pm0.231$	&$3.7$	&\rdelim\}{2}{20pt}[2.7]	&$18.2$\\
$20$	&SRP-24	&$1.000$	&$0$	&$0$	&$0$	&$6.729\pm0.237$	&$3.8$	&                       	&$23.8$\\
\midrule
$21$	&STEREO	&$1.000$	&$0$	&$0$	&$0$	&$6.340\pm0.159$	&$2.5$	&0	&$9-11$\\
$22$	&Chooz	&$0.496$	&$0.087$	&$0.351$	&$0.066$	&$6.117\pm0.191$	&$3.2$	&0	&$\approx 1000$\\
$23$	&Palo Verde	&$0.600$	&$0.070$	&$0.270$	&$0.060$	&$6.253\pm0.327$	&$5.4$	&0	&$\approx 800$\\
$24$	&Nucifer	&$0.926$	&$0.008$	&$0.061$	&$0.005$	&$6.666\pm0.667$	&$10.8$	&0	&$7.2$\\
$25$	&RENO	&$0.571$	&$0.073$	&$0.300$	&$0.056$	&$5.852\pm0.097$	&$1.6$	&0	&$\approx 411$\\
$26$	&Double Chooz	&$0.520$	&$0.087$	&$0.333$	&$0.060$	&$5.710\pm0.063$	&$1.1$	&0	&$\approx 415$\\
$27$	&DANSS	&$0.541$	&$0.073$	&$0.332$	&$0.055$	&$6.026\pm0.243$	&$4.1$	&0	&$10.9-12.9$\\
$28$	&Daya Bay	&$0.564$	&$0.076$	&$0.304$	&$0.056$	&$5.840\pm0.072$	&$1.2$	&0	&$\approx 578$\\
\end{tabular}

